Forget Unlearning: Towards True Data-Deletion in Machine Learning

Unlearning algorithms aim to remove deleted data's influence from trained models at a cost lower than full retraining. However, prior guarantees of unlearning in literature are flawed and don't protect the privacy of deleted records. We show that when users delete their data as a function of published models, records in a database become interdependent. So, even retraining a fresh model after deletion of a record doesn't ensure its privacy. Secondly, unlearning algorithms that cache partial computations to speed up the processing can leak deleted information over a series of releases, violating the privacy of deleted records in the long run. To address these, we propose a sound deletion guarantee and show that the privacy of existing records is necessary for the privacy of deleted records. Under this notion, we propose an accurate, computationally efficient, and secure machine unlearning algorithm based on noisy gradient descent.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/sec_tightness.tex <==
% !TEX root = ../main.tex

\section{Tightness of Unlearning} 
\label{sec:tightness}



==> sections/unlearn_convex.tex <==
% !TEX root = ../main.tex

\subsection{Data-deletion and accuracy guarantees under convexity}
\label{sec:unlrn_convex}

In this section we analyze data-deletion and utility guarantees for algorithm pair $(\Lrn_\Nsgd, \Unlrn_\Nsgd)$ when 
$\loss(\thet;\x)$ is convex and $\smh$-smooth. We fix the weight initialization distribution to 
$\rhO = \Gaus{0}{\frac{\noise^2}{\cvx(1-\step\cvx/2)}\Id}$ and define a mapping $\pI(\D)$ as 
%
\begin{equation}
	\label{eqn:pi_convex}
	\pI(\D) = \Nsgd(\D, \Ze, \K_u), \quad \text{where}\ \Ze \sim \rhO.
\end{equation}
%

To prove data-deletion as per our definition~\ref{dfn:unlearning}, we bound the R\'enyi divergence of unlearnt model 
$\hat\Thet_i$ with respect to distribution $\pI(\D_i)$ for all $i\geq 1$. Our proof is presented in two stages
(accompanined by several auxiliary lemmas in the appendix~\ref{app:proofs_unlrn} to help along the way) -- an information bound on the model followed by deletion of the records' information for any desired bound. In the first stage, 
we prove that there is an upper limit on the amount of information that a trained/unlearnt model $\hat\Thet_{i-1}$ can store. 
To be precise, we prove that $\Ren{\q}{\hat\Thet_{i-1}}{\rhO} = O(1)$ with respect to $i$. We show this by viewing the generation
process of the model $\hat\Thet_{i-1}$ as an extended run of Noisy SGD over changing databases. To trace how far
the Noisy SGD diverges from the weight initalization distribution $\rhO$, we construct a hypothetical Noisy SGD run
that is similar, except that its stationary distribution is $\rhO$ itself. By
interpolating the two Noisy SGD runs and tracing the rate of divergence between the two using results from
\citet{chourasia2021differential}, we are able to establish that the output distributions of the two are always
bounded in divergence.
%
\begin{theorem}[Information capacity of Noisy SGD]
	\label{thm:info_capacity}
	If weight initialization distribution is $\rhO = \Gaus{0}{\frac{\noise^2}{\cvx(1 - \step\cvx/2)}}$, loss 
	function $\loss(\thet;\x)$ is convex and $\smh$-smooth, and step size is $\step \leq \frac{2}{2\cvx + \smh}$, 
	then for all $i\geq 0$, the R\'enyi divergence of model $\hat\Thet_i$ w.r.t. a randomly intialized model 
	$\Ze \sim \rhO$ is 
	%
	\begin{equation}
		\Ren{\q}{\hat\Thet_i}{\Ze} < \frac{\q\lip^2}{\cvx\noise^2}.
	\end{equation}
\end{theorem}
%
This limit on capacity of model $\hat\Thet_i$ is an upper bound on the information content about the records to be deleted by
the edit request $\up_i$, which by itself constitutes a data-deletion guarantee for $(\Lrn_\Nsgd, \Unlrn_\Nsgd)$ 
with respect to the distribution $\rhO$. However, in the second stage, we show that the data-deletion algorithm $\Unlrn_\Nsgd$ 
updates the model $\hat\Thet_{i-1}$ to forget information about the records deleted by request $\up_i$ under any desired tolerance,
i.e., for any $\eps \geq 0$, enough deletion iterations $\K_u$ ensures $\Ren{\q}{\hat\Thet_i}{\pI(\D_i)} \leq \eps$.
We prove this by noting that both the distributions $\pI(\D_i)$ and that of unlearnt model $\hat\Thet_i$ are results of 
Noisy SGD runs over the same database $\D_i$. Therefore, the divergence between their respective weight initializations $\rhO$
and $\hat\Thet_{i-1}$ rapidly shrinks with every gradient descent step. Following theorem describes our data-deletion guarantee, 
along with its computational advantage over fresh retraining under an excess empirical risk constraint.
%
\begin{table}[t!]
	\caption{Comparision of computation savings in gradient complexity with prior $(\eps,\del)$-unlearning\protect\footnotemark~algorithms with excess risk upper bound of $\risk$. Edit requests
		modify $\reps=1$ record in $\n$-sized databases and model dimension is $\dime$. We assume batch size $\bsize = \n$, $\eps \leq 2 \log(1/\del)$ and loss $\loss(\thet;\x)$ to be $1$-Lipschitz and $O(1)$-smooth, 
		and $\ltwo$ regularization constant to be $O(1)$.}
	\label{tab:comparision}
	\centering
	\small
	\vspace{0.15cm}
	\begin{tabular}{|l|l|l|l|l|l|}
	\hline
	Algorithm                                    & Require secret states?      & Computation savings for $i$th edit                                          \\[0.14cm] \hline
	\multirow{2}{*}{\citet{neel2021descent}'s PGD}  & Yes, as per~\cite[Theorem 3.1]{neel2021descent}                         & $O\left(\log \left(\frac{\eps\n}{\sqrt\dime}\right)\right)$                 \\[0.14cm] \cline{2-3} 
						     & No, as per~\cite[Theorem 3.2]{neel2021descent}                          & $O\left(\log \left(\frac{\eps\n}{\log^2(i \dime)\sqrt\dime}\right)\right)$  \\[0.14cm] \hline
	Our Noisy-SGD   & No, as per Theorem~\ref{thm:unlearning_accuracy_convex}                          & $O\left(\log \left(\frac{\eps\n}{\sqrt\dime}\right)\right)$                 \\[0.14cm] \cline{1-3} 
	\end{tabular}
	\vspace{-0.28cm}
\end{table}
%
\footnotetext{\footnotesize From conversion~\cite[Proposition 3]{mironov2017renyi}, $(\q,\eps')$-R\'enyi divergence implies $(\eps, \del)$-indistinguishability for ${\q = 1 + \frac{2}{\eps} \log(1/\del)}$ and $\eps' = \eps/2$. When $\eps \leq 2 \log(1/\del)$, one can evaluate that $\frac{\q}{\eps'} \leq \frac{8 \log(1/\del)}{\eps^2}$.}
%
\begin{theorem}[Data-deletion, utility, and computational tradeoffs for Noisy SGD under convexity]
	\label{thm:unlearning_accuracy_convex}
	In the setting described in definition~\ref{dfn:noisy_sgd_unlrn}, suppose the loss 
	function $\loss(\thet;\x)$ is convex and $\smh$-smooth, and $\reg(\thet)$ is the $\ltwo(\cvx)$ regularizer, 
	initialization weight distribution is 
	$\rhO = \Gaus{0}{\frac{\noise^2}{\cvx(1 - \step\cvx/2)\Id}}$, batch size is $\bsize$, and step size is 
	$\step \leq \frac{1}{\cvx + \smh}$. 
	Let $\kappa = \frac{\cvx + \smh}{\cvx}$, and $\T \geq \frac{2}{\step\cvx} \log 4\kappa$.
	For any $\K_u \geq \T$, suppose the learning algorithm $\Lrn_\Nsgd$ is run for 
	$\K_p \geq \K_u + \frac{4}{\step\cvx} \log \frac{\n}{8\reps}$ steps, and for all edit requests $\up_i$ that modify 
	not more than $\reps$ records, the data-deletion algorithm $\Unlrn_\Nsgd$ run for $\K_u$ steps. 
	If, for some constants $\q > 1$ and $\eps > 0$,
	%
	\begin{equation}
		\noise^2 = \frac{\q\lip^2}{\eps\cvx}\exp\left(-\frac{\cvx\step\K_u}{2}\right),
	\end{equation}
	%
	then, the algorithm pair $(\Lrn_\Nsgd, \Unlrn_\Nsgd)$ satisfies perfect $(\q, \eps)$-data-deletion, and for all $i\geq0$, the models $\hat\Thet_i$ have an excess empirical risk of
	%
	\begin{equation}
		\label{eqn:induction_excess_risk}
		\err(\hat\Thet_i;\D_i) \leq 2\noise^2\left(\frac{4\eps\reps^2}{\q\n^2} + \kappa\dime\right) + \frac{\step\kappa\lip^2(\n - \bsize)}{\bsize\n}.
	\end{equation}
	%
\end{theorem}
%
A formal proof of theorem~\ref{thm:info_capacity} and theorem~\ref{thm:unlearning_accuracy_convex} can be found in appendix
\ref{app:proofs_unlrn}. For our excess risk analysis, we prove and make use of the following convergence guarantee.
%
\begin{theorem}[Excess empirical risk of Noisy SGD]
	\label{thm:excess_risk_convex}
	For convex and $\smh$ smooth loss function $\loss(\thet;\x)$, if step size $\step \leq \frac{1}{\cvx+\smh}$, the excess empirical risk of 
	$\Thet_\K = \Nsgd(\D, \Thet_0, \K)$, is bounded as
	\begin{equation}
		\err(\Thet_\K;\D) \leq \err(\Thet_0;\D)e^{-\cvx\step\K} + \left(1 + \frac{\smh}{\cvx}\right)\left[\frac{\step\lip^2(\n - \bsize)}{2\bsize\n} + \dime\noise^2\right].
	\end{equation}
\end{theorem}





==> sections/unlearn_nonconvex.tex <==
% !TEX root = ../main.tex

\subsection{Data-deletion guarantees under non-convexity}
\label{sec:unlrn_nonconvex}
Data-deletion guarantees need to hold under practical scenarios. Most applications of machine learning today tend to have non-convex loss functions and we are the first to provide a theoretical guarantee for data-deletion (or even unlearning) under this setting. To simulate standard training procedures we consider batch sub-sampling to be a part of Noisy SGD.
We provide data-deletion and utility guarantee for $(\Lrn_\Nsgd, \Unlrn_\Nsgd)$ when loss function 
$\loss(\thet;\x)$ is non-convex but bounded and $\smh$-smooth. The mapping $\pI(\D)$ that we show data-deletion
with respect to is the Gibbs distribution defined as
\begin{equation}
	\label{eqn:lrn_alg}
	\pI(\D)(\thet) \propto e^{-\rLoss_{\D}(\thet) / \noise^2}.
\end{equation}
%
Recall that this Gibbs distribution is equivalent to the Bayesian posterior. First order gradient descent based sampling algorithms
like Langevin Monte Carlo, Stochastic Gradient Langevin Diffusion, etc., outputs samples that approximate this Bayesian posterior.
The quality of approximation has been widely studied in literature in form of convergence guarantees in various divergence notions
such as Wasserstein distance~\cite{dalalyan2019user,dalalyan2017further}, 
KL-divergence~\cite{vempala2019rapid,dalalyan2017theoretical}, $\chi^2$-divergence~\cite{erdogdu2022convergence}, and R\'enyi
divergence~\cite{wibisono2019proximal,vempala2019rapid}. Of special interest to us is \citet{chewi2021analysis}'s convergence
analysis of Unadjusted Langevin Algorithm (ULA) in R\'enyi divergence under mild isoperimetric assumptions on the 
Bayesian posterior. The Noisy SGD algorithm is similar to ULA and we aim to prove data-deletion with respect
to the Bayesian posterior itself. However, to account for gradient clipping and stochastic mini-batches we extend their results and presented in the following theorem is our extension of convergence 
\cite[Theorem 4]{chewi2021analysis} to the setting of Noisy SGD.
%
\begin{theorem}[Convergence of Noisy SGD in R\'enyi divergence]
	\label{thm:convergence}
	Let constants $\lip, \smh \geq 0$, $\cvx \leq 512$, and $\q, \B > 1$. Suppose the initial weights ${\Ze \sim \rhO 
	 = \Gaus{0}{\frac{\noise^2}{\cvx}\Id}}$, the loss function $\loss(\thet;\x)$ is $(\noise^2\log(\B)/4)$-bounded, 
	and $\smh$-smooth, and $\reg(\thet)$ is the $\ltwo(\cvx)$ regularizer. If step size 
	is ${\step \leq \frac{\cvx}{128\B\q^2(\smh + \cvx)^2}}$, then for any database $\D \in \X^\n$, the R\'enyi divergence
	of output model $\Thet_{\step \K} = \Nsgd(\D, \Ze, \K)$ with respect to the Gibbs distribution $\pI(\D)$ defined in
	\eqref{eqn:lrn_alg} shrinks as follows:
	%
	\begin{equation}
		\Ren{\q}{\Thet_{\step \K}}{\pI} \leq \q\exp\left( - \frac{\cvx\step\K}{2\B} \right) \Ren{\q}{\Ze}{\pI} + \frac{32 \B \q}{\cvx} \left(\frac{\lip^2}{\noise^2} + 2\dime\step(\smh+\cvx)^2\right).
	\end{equation}
	%
\end{theorem}
%
Though the proof is alike to~\citet{chewi2021analysis}( presented in 
appendix~\ref{sec:noisysgd_convergence}).], our solution to the differential inequations is slightly tighter, resulting in
a $\log(\q)$ improvement asymptotically as well as the aforementioned extensions for Noisy SGD.


In contrast with the analysis approach in section~\ref{sec:unlrn_convex}, we argue both utility and data-deletion properties of 
$(\Lrn_\Nsgd, \Unlrn_\Nsgd)$ through the proximity of unlearnt models $\hat\Thet_i$ to the Gibbs posterior $\pI(\D_i)$ by
virtue of the rapid convergence theorem~\ref{thm:convergence}. Since our definition of excess empirical risk $\err(\hat\Thet_i;\D_i)$ 
in this setting is the loss difference in expectation with respect to $\pI(\D_i)$, the utility guarantee is a direct by-product 
of the indistinguishability between the two distributions.
%
\begin{theorem}[Data-deletion, utility, and computational tradeoffs for Noisy SGD under non-convexity]
	\label{thm:unlearning_nonconvex}
	In the setting described in definition~\ref{dfn:noisy_sgd_unlrn}, suppose the weight distribution is
	$\rhO = \Gaus{0}{\frac{\noise^2}{\cvx}\Id}$, loss function $\loss(\thet;\x)$ is 
	$\frac{\noise^2\log(\B)}{4}$-bounded and $\smh$-smooth, $\reg(\thet)$ is the $\ltwo(\cvx)$ regularizer, and step 
	size is $\step$. If for some constants $\q > 1$ and $\eps \geq 0$,
	%
	\begin{align}
		\step \leq \frac{\cvx\eps}{256\dime\q\B(\smh+\cvx)^2}, \quad\quad&\text{and}\quad\quad \noise^2 \geq \frac{128\B\q\lip^2}{\cvx \epsilon},
	\end{align}
	%
	then running the learning algorithm $\Lrn_\Nsgd$ for ${\K_p}$ iterations, followed by running data-deletion algorithm 
	$\Unlrn_\Nsgd$ for $\K_u$ iterations per edit request $\up_i$ satisfies $(\q, \eps)$ R\'enyi data-deletion, and
	has an excess empirical risk $\err(\hat\Thet_i;\D_i) \leq \eps\B\noise^2(1 + \smh/\cvx) + \tilde O(\dime \noise^2)$,
	%
	% \begin{enumerate}
	% 	\item perfect $(\q, \eps)$ R\'enyi unlearning, and
	% 	\item has an excess empirical risk $\err(\hat\Thet_i;\D_i) \leq \eps\B\noise^2(1 + \smh/\cvx)$,
	% \end{enumerate}
	%
	whenever
	\begin{align}
		\K_p \geq \frac{2\B}{\cvx\step} \log \frac{\q\log(\B)}{\eps}, \quad\quad& \K_u \geq \K_p - \frac{2\B}{\cvx\step}\log \left(\frac{\log(\B)}{2\left(\eps + \frac{\reps}{\n} \log(\B) \right)}\right).
	\end{align}
\end{theorem}

From the above theorem, we observe a strict computational benefit in data-deletion, whenever the fraction of edited records in a 
single update request satisfies $\frac{\reps}{\n} \leq \frac{1}{2} - \frac{\eps}{\log \B}$. In the high privacy regime 
where $\eps \leq \frac{\reps}{\n}\log(\B)$, relying on data-deletion rather than fresh learning is $O(\log (\n/4\reps))$ cheaper. 

%Furthermore, the number of steps required to guarantee unlearning is independent of the length of the edit sequence. The convergence guarantee results in the output of the unlearning algorithm to be within a bounded risk value for every iteration, independent of the specific iteration itself. Thus, our unlearning guarantee can be considered \emph{strong}, by definition.





% In deviation to prior works, our learning algorithm isn't gradient-descent based, rather is a (computationally intractable) exact 
% sampling algorithm. The output of the learning algorithm serves as a distribution that is independent of deleted data-records, and 
% therefore showing indistinguishability of the unlearning algorithm's output w.r.t. this distribution ensures unlearning. Being a
% pen-and-paper proof, infeasiblity of learning algorithm isn't a concern as only the unlearning algorithm is ever executed. 
% As for the inital model $\hat\Thet_0$, our unlearning guarantee requires it to be only sufficiently close to the $\Lrn(\D_0)$, and
% can therefore be approximated via Noisy SGD.

% The secondary role of the learning algorithm is to argue about the computational savings afforded on using an unlearning algorithm 
% instead of fresh learning. Since our learning algorithm is intractable, we argue the computational advantage of unlearning via 
% Noisy SGD via directly comparing it to a fresh learn using Noisy SGD and performing other baseline experiments.

% Our unlearning results are inspired by \citet{chewi2021analysis}'s rapid convergence results of Langevin Monte Carlo algorithms
% in R\'enyi divergence. By showing a similar rate of convergence for Noisy SGD, we argue along the lines of \citet{neel2021descent}
% that descent-to-delete makes a pre-trained model quickly forget deleted records.


% \subsection{Unlearning Guarantee for Noisy SGD}
% 
% In this section, we utilyze the convergence guarantee to prove that Noisy SGD is a perfect unlearning algorithm with respect
% to the learning algorithm $\Lrn$ that samples from the Gibbs distribution. 
% 
% Our overarching intuition is straightforward and we attempt the proof by induction. Consider the unlearning algorithm is at it's $i^{th}$ step. It begins from a point close to the optima of the $i-1^{th}$ step (which is the metadata it has received and forms the induction hypothesis). 
% We bound the distance between the optima of $i^{th}$ and $i-1^{th}$ step (as seen in \ref{eqn:optima_bound}). We use the triangle inequality (\ref{triangle_inequality}) to obtain the distance between the starting point (output $i-1^{th}$ step) and the target (optima of $i^{th}$ step). Using the above bound we then rely on our convergence result (\ref{thm:convergence}) to guarantee reaching sufficiently close to the optima, within a fixed number of steps. Our notable contribution here lies not only in orchestrating these disparate notions into a unified harmony but also extending the previously proven convergence result to consider batch-sub sampling, gradient clipping and arbitrary noise scaling.
 

% Note that the asymptotic constant of the convergence guarantee has a linear dependence on dimension $\dime$. To mitigate it, we
% set the value of step size $\step$ to be of the order $\frac{1}{\dime}$. This helps ensure that the unlearning $\eps$ values under 
% consideration accord practical benefits and defenses against an adversary.
% 
% The number of steps needed for each unlearning iteration is inversely influenced by the regularizer $\lambda$, step size $\step$, and the indistinguishability guarantee $\eps$. This is in line with our intuition as we would expect the number of steps to decrease as the regularization increases (the function becomes less non convex), the step size increases (we converge to the optima faster) and $\eps$ increases (we have a lower privacy threshold).

